Cross-Input Certified Training for Universal Perturbations

Existing work in trustworthy machine learning primarily focuses on single-input adversarial perturbations. In many real-world attack scenarios, input-agnostic adversarial attacks, e.g. universal adversarial perturbations (UAPs), are much more feasible. Current certified training methods train models robust to single-input perturbations but achieve suboptimal clean and UAP accuracy, thereby limiting their applicability in practical applications. We propose a novel method, CITRUS, for certified training of networks robust against UAP attackers. We show in an extensive evaluation across different datasets, architectures, and perturbation magnitudes that our method outperforms traditional certified training methods on standard accuracy (up to 10.3\%) and achieves SOTA performance on the more practical certified UAP accuracy metric.

==> contents/old/3-technical_contribution.tex <==
\section{Certified Training for Universal Perturbations}

In this section, we introduce for formal training objective for UAP robustness and the intuition for \method.

\subsection{UAP Training Objective}

Equation \ref{eq:trainrob} gives the training objective for standard single-input adversarial robustness: minimizing the expected value of the effect of a single-input adversarial perturbation. For UAP robustness, we minimize the loss coming from a single universal perturbation.

\begin{equation} \label{eq:uaptrainrob}
    \theta = \argmin_\theta \max_{\mathbf{u}\in \mathcal{B}(0,\epsilon)}\left(\mathop{\mathbb{E}}_{(x,y) \in \mathcal{X}}\left[ \mathcal{L}_f(\mathbf{x} + \mathbf{u}, y)\right]\right)
\end{equation}

Here, since UAPs are input-agnostic we do the inner maximization outside of the expectation. Next, we introduce the idea of $k$-common perturbations, show how they relate to Equation \ref{eq:uaptrainrob}, and use them to derive a key theorem for upperbounding Equation \ref{eq:uaptrainrob}.
%Above we show that IBP is used over-approximate the inner maximization for certified training. The adversarial robustness objective can be achieved directly from the output of the bound propagation. Current SOTA methods for worst-case UAP accuracy verification use a combination of linear relaxation and MILP solving which is non-differentiable and thus not easily converted to a loss function; we leave this application to future work. 



\subsection{$k$-Common Perturbations}

An adversarial perturbation, $\mathbf{u}$, is a $k$-common perturbation ($k$-cp) if it causes at least $k$ inputs to misclassify. Let's first define an indicator function, $A_f:\mathbb{R}^{\din}\times\mathbb{R} \to \{1, 0\}$ for if $f$ is adversarial for $\mathbf{x}, y$:

\begin{equation*}
A_f(\mathbf{x}, y) = 
\begin{cases}
    1 &\text{ if } \hat{f}(\mathbf{x}) \neq y\\
    0 &\text{ otherwise}
\end{cases}
\end{equation*}

Formally, $\mathbf{u}$ is a $k$-common perturbation on data distribution $\mathcal{X}$ for network $f$, if $\exists \{(\mathbf{x}_i, y_i)|i\in [k]\} \in \mathcal{X}^k. \min(A_f(\mathbf{x}_1 + \mathbf{u}, y_1), \dots, A_f(\mathbf{x}_k + \mathbf{u}, y_k)) = 1$. Note that by this definition a $k$-cp is also a $(k-1)$-cp, $\dots$, $1$-cp. Next, define $\Psi_{\mathcal{X}, f}(k, \epsilon):\mathbb{Z}\times\mathbb{R} \to \{1,0\}$ as

\begin{equation*}
\Psi_{\mathcal{X}, f}(k,\epsilon) = 
\begin{cases}
    1 & \text{ if } \exists \mathbf{u}\in \mathcal{B}(\mathbf(0), \epsilon), \{(\mathbf{x}_i,y_i)|i\in [k]\} \in \mathcal{X}^k.\\
    & \hspace{20pt}\min(A_f(\mathbf{x}_1 + \mathbf{u}, y_1), \dots, A_f(\mathbf{x}_k + \mathbf{u}, y_k)) = 1\\
    0 & \text{ otherwise}
\end{cases}
\end{equation*}

In other words, $\Psi_{\mathcal{X}, f}(k, \epsilon)$ indicates if a $k$-common perturbation exists on $\mathcal{X}$ for $f$. Further, define $\Psi_{\mathcal{X}, f}(0,\epsilon) = 1$ and $\Psi_{\mathcal{X}, f}(|\mathcal{X}| + 1,\epsilon) = 0$ as edge cases. Note that $\forall j>k.\Psi_{\mathcal{X}, f}(k, \epsilon)=0 \implies \Psi_{\mathcal{X}, f}(j, \epsilon) = 0$. Let $\kappa_{\mathcal{X}, f}$ be the largest number of inputs that can be misclassified by a single perturbation. Since $\Psi$ is binary and monotonic in $k$ we know that there must exist a singular transition point from $1$ to $0$. Formally, let $\kappa_{\mathcal{X}, f}$ be s.t. $\Psi_{\mathcal{X}, f}(\kappa_{\mathcal{X}, f}, \epsilon) = 1$ and $\Psi_{\mathcal{X}, f}(\kappa_{\mathcal{X}, f} + 1, \epsilon) = 0$. Let's assume that we use $A_f$ as a loss $\mathcal{L}_f$ for Equation \ref{eq:uaptrainrob}, then we have
\begin{lemma}\label{lm:kuap}
Given data distribution $\mathcal{X}$ and network $f$
\begin{equation}
    \max_{\mathbf{u}\in \mathcal{B}(0,\epsilon)}\left(\mathop{\mathbb{E}}_{(\mathbf{x},y)\in \mathcal{X}}\left[ A_f(\mathbf{x} + \mathbf{u}, y)\right]\right) = \frac{1}{|\mathcal{X}|}\sum^{|\mathcal{X}|}_{i=1} \Psi_{\mathcal{X}, f}(i,\epsilon)
\end{equation}
\end{lemma}

\begin{proof}
On the LHS, we are finding the worst-case proportion of inputs affected by a single perturbation, formally, $\max_{\mathbf{u}\in \mathcal{B}(0,\epsilon)}\left(\mathop{\mathbb{E}}_{(\mathbf{x},y)\in \mathcal{X}}\left[ A_f(\mathbf{x} + \mathbf{u}, y)\right]\right) = \frac{\kappa_{\mathcal{X}, f}}{|\mathcal{X}|}$.
\begin{align*}
    \frac{1}{|\mathcal{X}|}\sum^{|\mathcal{X}|}_{i=1} \Psi_{\mathcal{X}, f}(i,\epsilon) &= \frac{1}{|\mathcal{X}|}\left(\sum^{\kappa_{\mathcal{X}, f}}_{i=1} \Psi_{\mathcal{X}, f}(i,\epsilon) + \sum^{|\mathcal{X}|}_{i=\kappa_{\mathcal{X}, f} + 1} \Psi_{\mathcal{X}, f}(i,\epsilon)\right)\\
    &= \frac{1}{|\mathcal{X}|}\left(\sum^{\kappa_{\mathcal{X}, f}}_{i=1} 1 + \sum^{|\mathcal{X}|}_{i=\kappa_{\mathcal{X}, f} + 1} 0\right) = \frac{\kappa_{\mathcal{X}, f}}{|\mathcal{X}|} && (\text{by definition of }\kappa)\\
    & = \max_{\mathbf{u}\in \mathcal{B}(0,\epsilon)}\left(\mathop{\mathbb{E}}_{(\mathbf{x},y)\in \mathcal{X}}\left[ A_f(\mathbf{x} + \mathbf{u}, y)\right]\right)
\end{align*}
\end{proof}


%On the LHS, we are finding the worst-case proportion of inputs affected by a single perturbation, $\frac{\kappa}{|\mathcal{X}|}$. On the RHS, $\forall 1\leq i\leq \kappa. \Psi_{\mathcal{X},f}(i,\epsilon) = 1$ and $\forall i\geq \kappa. \Psi_{\mathcal{X},f}(i,\epsilon) = 0$, therefore,  \ref{eq:uaptrainrob} is minimized when there exists no adversarial perturbations for any input, in other words, $\nexists$ $1$-UAP. More specifically, we can write

Next, we give a corollary which builds to the main theorem (\ref{th:robuap}) behind \method. 

\begin{corollary}\label{cor:kuap} Given data distribution $\mathcal{X}$ and network $f$, $\forall k \in \mathbb{Z}^{+}$
    $$\frac{1}{|\mathcal{X}|}\sum^{|\mathcal{X}|}_{i=k} \Psi_{\mathcal{X}, f}(i,\epsilon) \leq \mathop{\mathbb{E}}_{\{(x_i,y_i) |i\in [k]\} \in \mathcal{X}^k} \left[\max_{\mathbf{u}\in\mathcal{B}(\mathbf{0},\epsilon)} \min(A_f(\mathbf{x}_1+\mathbf{u}, y_1), \dots, A_f(\mathbf{x}_k+\mathbf{u},y_k))\right]$$
\end{corollary}

\begin{proof}
    We split our proof based on $\kappa_{\mathcal{X}, f}$
    \begin{case}
        $\kappa_{\mathcal{X}, f} < k$ 
    \end{case}
    $\forall i>\kappa_{\mathcal{X}, f}. \Psi_{\mathcal{X}, f}(i,\epsilon) = 0$, so the LHS equals 0 and the RHS is non-negative.
    \begin{case}
        $\kappa_{\mathcal{X}, f} = k$ 
    \end{case}
    $\Psi_{\mathcal{X}, f}(\kappa_{\mathcal{X}, f},\epsilon) = 1$ and $\Psi_{\mathcal{X}, f}(\kappa_{\mathcal{X}, f} + 1,\epsilon) = 0$ by definition of $\kappa$. So the LHS of the inequality equals $\frac{1}{|\mathcal{X}|}$. Furthermore, by definition of $\Psi$, $\exists \mathbf{u}\in \mathcal{B}(\mathbf(0), \epsilon), \{(\mathbf{x}_i,y_i)|i\in [\kappa_{\mathcal{X}, f}]\} \in \mathcal{X}^{\kappa_{\mathcal{X}, f}} \min(A_f(\mathbf{x}_1 + \mathbf{u}, y_1), \dots, A_f(\mathbf{x}_k + \mathbf{u}, y_k)) = 1 \implies \text{RHS}\geq \frac{1}{|\mathcal{X}|}$
    \begin{case}
        $\kappa_{\mathcal{X}, f} > k$ 
    \end{case}
    LHS equals $\frac{\kappa_{\mathcal{X}, f} - k + 1}{|\mathcal{X}|}$ as $\forall i\leq\kappa_{\mathcal{X}, f}. \Psi_{\mathcal{X}, f}(i,\epsilon) = 1$ by definition of $\kappa$. By definition of $\Psi$, $\exists \mathbf{u}\in \mathcal{B}(\mathbf(0), \epsilon), \{(\mathbf{x}_i,y_i)|i\in [\kappa_{\mathcal{X}, f}]\} \in \mathcal{X}^{\kappa_{\mathcal{X}, f}} \min(A_f(\mathbf{x}_1 + \mathbf{u}, y_1), \dots, A_f(\mathbf{x}_k + \mathbf{u}, y_k)) = 1$. This implies there is a set of $\kappa_{\mathcal{X}, f}$ inputs which are all misclassified when added to some common perturbation, $\mathbf{u}$. There are ${\kappa \choose k}$ sets of $k$ inputs taken from this set which are all misclassified when added to $\mathbf{u}$. Therefore, $\text{RHS} \geq {\kappa \choose k}/|\mathcal{X}| \geq \frac{\kappa_{\mathcal{X}, f} - k + 1}{|\mathcal{X}|}$ = \text{LHS}.
\end{proof}

We can now get our core theorem which allows us to upper bound the UAP robustness objective with the proportion of tuples which contain a $k$-cp.

\begin{theorem}\label{th:robuap}
Given data distribution $\mathcal{X}$ and network $f$, $\forall k \in \mathbb{Z}^{+}$
\begin{align*}
    \max_{\mathbf{u}\in \mathcal{B}(0,\epsilon)}\left(\mathop{\mathbb{E}}_{(\mathbf{x},y)\in \mathcal{X}}\left[ A_f(\mathbf{x} + \mathbf{u}, y)\right]\right)\leq& \mathop{\mathbb{E}}_{\{(x_i,y_i) |i\in [k]\} \in \mathcal{X}^k} \Bigl[\max_{\mathbf{u}\in\mathcal{B}(\mathbf{0},\epsilon)} \min(A_f(\mathbf{x}_1+\mathbf{u}, y_1),\\
    &\dots, A_f(\mathbf{x}_k+\mathbf{u},y_k))\Bigr]+ \frac{1}{|\mathcal{X}|}\sum_{i=1}^{k-1} \Psi_{\mathcal{X}, f}(i,\epsilon)
\end{align*}
\end{theorem}

\begin{proof}
\begin{align*}
    \max_{\mathbf{u}\in \mathcal{B}(0,\epsilon)}&\left(\mathop{\mathbb{E}}_{(\mathbf{x},y)\in \mathcal{X}}\left[ A_f(\mathbf{x} + \mathbf{u}, y)\right]\right)= \frac{1}{|\mathcal{X}|}\sum^{|\mathcal{X}|}_{i=1} \Psi_{\mathcal{X}, f}(i,\epsilon) && (\text{by Lemma \ref{lm:kuap}})\\
    &= \frac{1}{|\mathcal{X}|}\sum^{|\mathcal{X}|}_{i=k} \Psi_{\mathcal{X}, f}(i,\epsilon) + \frac{1}{|\mathcal{X}|}\sum^{k-1}_{i=1} \Psi_{\mathcal{X}, f}(i,\epsilon)\\
    &\leq \mathop{\mathbb{E}}_{\{(x_i,y_i) |i\in [k]\} \in \mathcal{X}^k} \Bigl[\max_{\mathbf{u}\in\mathcal{B}(\mathbf{0},\epsilon)} \min(A_f(\mathbf{x}_1+\mathbf{u}, y_1), \\
    &\dots, A_f(\mathbf{x}_k+\mathbf{u},y_k))\Bigr] + \frac{1}{|\mathcal{X}|}\sum^{k-1}_{i=1} \Psi_{\mathcal{X}, f}(i,\epsilon) && (\text{by Corollary \ref{cor:kuap}})
\end{align*}
\end{proof}

Theorem \ref{th:robuap} tells us that the inner maximization for the UAP training objective can be upperbounded by the proportion of tuples that have a $k$-cp and indicators for $j$-cp for $j<k$. In the next section, we will explore how we use this fact as the core intuition for \method.
%overapproximated by the sum of two terms: a loss based on $2$-UAPs and an indicator for $1$-UAPs. Given the existing research on the hardness and over-regularization coming from minimizing $1$-UAPs, if we assume that their exists $1$-UAPs then we can take the last term as a constant and not regularize for it and instead train to be robust against $2$-UAPs. This is the key insight for \method. 

%If a network contained no single-input adversarial perturbations for a ball, $\mathcal{B}(0,\epsilon)$, then there also does not exist any UAPs on the same ball. While we would ideally like to train a network that satisfies the above, existing research has already shown the difficulty of that problem. For worst-case UAP accuracy, the next best scenario is that there only exists single-input adversarial perturbations.

\section{\method}

In the previous section, we explored the UAP robustness training objective. In this section, we will use what we learned to develop an algorithm for certified training for UAPs.

\subsection{\method Loss}

%The core problem at the heart of robust training is balancing regularization coming from the robust loss term. Adversarial training does not incur enough regularization and thus gets poor certified accuracy while certified training over regularizes and gets suboptimal accuracy. \method aims to lower the regularization cost as it only aims to be certifiably robust for universal perturbations.



Theorem \ref{th:robuap} gives us that the UAP robustness objective can overapproximated by considering only $2$-UAPs. For a single input, $x_i$, coming from batch $\mathcal{X}_B$, we can ensure that there are no $2$-UAPs involving $x_i$ if the adversarial regions for other inputs in the batch are not adversarial for $x_i$. Since we can not get the precise adversarial regions, we approximate these regions using small boxes around single adversarial perturbations. Formally, given a batch of inputs, $\mathcal{X}_B = \{\mathbf{x}_1, \mathbf{x}_2, \dots, \mathbf{x}_m\}$, and ball $\mathcal{B}(0,\epsilon)$ we first find adversarial perturbations, $\mathbf{v}_1, \mathbf{v}_2, \dots, \mathbf{v}_m$, for each input within a truncated ball $\mathcal{B}(0, \epsilon - \tau)$. With this, we can give our loss for input $i$ in $\mathcal{X}_B$ as

\begin{equation}
    \mathcal{L}_{\text{\method}}(\mathcal{X}_B, i, \epsilon, \tau) \coloneqq \sum_{j \in [m], j\neq i} \mathcal{L}_{\text{IBP}}(\mathbf{x}_i + \argmax_{\mathbf{v} \in \mathcal{B}(\mathbf{0}, \epsilon - \tau)} \mathcal{L}(\mathbf{x}_j,y_j) , y_i, \tau) 
\end{equation}

In practice, when computing this loss over an entire batch, we can precompute adversarial perturbations (the inside argmax) as each perturbation will be used for all other inputs in the batch.



% <fix>

% \begin{equation}\label{eq:advvsuap}
%     \max_{\mathbf{v}\in \mathcal{B}(0,\epsilon)}\left(\mathop{\mathbb{E}}_{x,y}\left[ \mathcal{L}(\mathbf{x} + \mathbf{v}, y)\right]\right) \leq \mathop{\mathbb{E}}_{\mathbf{x}, y}\left[ \max_{\mathbf{x'} \in \mathcal{B}(\mathbf{x}, \epsilon)} \mathcal{L}(\mathbf{x}', y)\right]
% \end{equation}

% The LHS computes the number of inputs affected by a single perturbation whereas the RHS computes the number of inputs that can be adversarially attacked on a per-input basis. A consequence of this is if the RHS of Equation \ref{eq:advvsuap} (the inner expectation from Equation \ref{eq:trainrob}) is $0$ then the LHS must also be $0$. While this is an ideal state, a $1$-UAP is also just a single-input adversarial perturbation and existing certified training research [cite] has already shown the significant regularization costs associated with optimizing for this problem. \method focuses on $2$-UAPs, we first prove the following corollary to give us a theoretical result.








\begin{figure*}[t]
    \centering
\includegraphics[width=1\textwidth]{images/certuap_intuition.png}
    \caption{Intuition behind \method. UAPs occur where adversarial regions ($\redbox$) from multiple inputs overlap ($\darkredbox$). To approximate this, adversarial examples ($\star$) are computed for each input, $x_i$, the corresponding perturbation vectors, $v_i$, (dark gray arrow <>) and adversarial regions are collocated to the perturbation space, $\mathcal{B}(\mathbf{0}, \epsilon)$. To overapproximate $\darkredbox$ we take cross-input adversarial perturbations and draw $l_\infty$ balls around them, $b_{i,j}^0 = \mathcal{B}(\mathbf{x}_i + \mathbf{v}_j, \tau)$.}
    \label{fig:intuition}
\end{figure*}

\subsection{Universal Perturbation Regions}

Figure \ref{fig:intuition} provides a simplified example to aid visual intuition. Given a batch of inputs $\mathcal{X}_B = \{\mathbf{x}_0, \mathbf{x}_1, \dots, \mathbf{x}_m\}$ and $l_\infty$-balls around each, $\mathcal{B}(\mathbf{x}_0, \epsilon), \dots, \mathcal{B}(\mathbf{x}_m, \epsilon)$. The light red regions, which we will refer to as \textit{adversarial regions} ($\redbox$) represent the portion of $\mathcal{B}(\mathbf{x}_i, \epsilon)$ which is adversarial for $\mathbf{x}_i$, the green regions ($\greenbox$) represent the portion which is correctly classified. Note that practically it is generally intractable to compute these exact regions [cite provably robust]. Instead, we can compute adversarial examples ($\star$) and their corresponding adversarial perturbations, $\mathbf{v}_0, \dots, \mathbf{v}_m$ (gray arrows <>). These computations occur in the input space; however, we can collocate all of the adversarial perturbations and adversarial regions around the origin (shown on LHS of Figure \ref{fig:intuition}). Ideally, for UAP robustness we want to train to be robust for regions where multiple inputs adversarial regions overlap ($\darkredbox$); however, these exact regions are intractable as they are intersections of the precise adversarial regions which themselves are intractable to compute. For a given input, another way to approximate the adversarial overlap regions is to 

This is the key insight of \method. 
%We model the adversarial region for other inputs, $\mathbf{x}_j$, by creating a small ball around the current input added to an adversarial perturbation computed from each other input, $\mathcal{B}(x_i + v_j, \tau)$. By doing this, we aim to capture the overlap regions while incurring less regularization, this will be further covered below.


\begin{figure*}[t]
    \centering
\includegraphics[width=1\textwidth]{images/certuap_propagation.png}
    \caption{Propagation for $\mathbf{x}_0$ and bounding boxes $b_{0,1}^0$ and $b_{0,m}^0$. The boxes are propagated using IBP through each layer of the network. In the output layer, we see that although $b_{0,m}^n$ does not capture the entire adversarial region for $\mathbf{x}_0$ it does capture the overlapping adversarial region between $\mathbf{x}_0$ and $\mathbf{x}_m$. Compared to IBP propagation ($\dashedbox$) we induce much less regularization (big blue <> vs. small blue <>). Depending on the size of the overlap region, SABR ($\color{gray}{\dashedbox}$) incurs more regularization (medium blue <>).}
    \label{fig:propagation}
\end{figure*}

\subsection{Propagation of Cross-Input Boxes}

We illustrate the propagation process for one input, $\mathbf{x}_0$, in Figure \ref{fig:propagation}. All boxes can be propagated through the network using any symbolic propagation method, but similarly to SABR we use \textsc{Box} propagation [cite] for its speed and well-behaved optimization problem [cite]. The output space visualizes the propagation of the cross-input adversarial boxes ($\square$) and the single-input adversarial, or SABR, box ($\color{gray}{\dashedbox}$). The dark red region ($\darkredbox$) represents the $2$-UAP overlap region between $\mathbf{x}_0$ and $\mathbf{x}_1$, we can see that at the end of the propagation $b_{0,1}^n$ includes the entire overlap region even though it does not include the entire adversarial region for $\mathbf{x}_0$. As a result of this, \method incurs less regularization (medium blue <> vs. small blue <>) compared to SABR propagation and significantly less than IBP propagation (big blue <>).

\subsection{Exclusion of Same-Input Adversarial Boxes}

Figure \ref{fig:propagation} gives us some insight into why we do not propagate an adversarial box on the input it comes from. SABR captures an unsound but much more precise region ($\color{gray}{\dashedbox}$) than IBP; however, for UAPs, we do not care that individual adversarial regions exist rather that there are no common regions shared among many inputs. Thus, for the UAP threat model, SABR's box is still over-regularizing (medium blue <>), \method captures the universal adversarial region while incuring less regularization. 

Theorem \ref{th:robuap} shows us that the UAP loss can be overapproximated by a term for $2$-UAP loss and a term for $1$-UAP loss. <add data for comparing the loss terms>

\subsection{\method Algorithm}

In Algorithm \ref{alg:algorithm}, we layout the framework for \method training. For each batch, $\mathcal{X}_B$, we first compute a set of adversarial perturbations $\mathbf{v}_i$ for each input $\mathbf{x}_i \in \mathcal{X}_B$ (Line 4). We then iterate through each input in the batch, $\mathbf{x}_i$ and through each cross-input adversarial perturbation, $\mathbf{v}_j$, not coming from the current input ($i\neq j$). We then update the loss by computing the IBP loss on a box centered at $\mathbf{x}_i + \mathbf{v}_j$ with radius $\tau$ (Line 8).

\begin{algorithm}[t]
   \caption{\method Algorithm}
   \label{alg:algorithm}
\begin{algorithmic}[1]
   \STATE Initialize $\theta$
   \FOR{\# of Epochs}
   \FOR{$\mathcal{X}_B \subset \mathcal{X}$}
        \STATE Compute $v_i$ adversarial perturbation for $x_i \in \mathcal{X}_B$
        \STATE $L_{\text{\method}} \gets 0$
        \FOR{$i \in |\mathcal{X}_B|$}
            \FOR{$j \in |\mathcal{X}_B| \& j \neq i$}
                \STATE $L_{\text{\method}} = L_{\text{\method}} + L_{\text{IBP}}(\mathbf{x}_i + \mathbf{v}_j, y_i, \tau)$
            \ENDFOR
        \ENDFOR
        \STATE Update $\theta$ using $L_{\text{\method}}$
   \ENDFOR
   \ENDFOR
\end{algorithmic}
\end{algorithm}

% The core problem at the heart of robust training is balancing regularization coming from the robust loss term. Adversarial training does not incur enough regularization and thus gets poor certified accuracy while certified training over regularizes and gets suboptimal accuracy. \method aims to lower the regularization cost as it only aims to be certifiably robust for universal perturbations. For a given input, $\mathbf{x}_i$, we do not need to train for its own adversarial perturbation, $\mathbf{v}_i$; instead, we will train the model so that $\mathbf{x}_i$ is robust for adversarial perturbations coming from $\mathbf{x}_1, \dots \mathbf{x}_{i-1}, \mathbf{x}_{i+1}, \mathbf{x}_m$. In practice, because of the 'black-box' nature of DNNs we can not get the precise adversarial regions for each input. Instead, we estimate these regions using small bounding boxes, $b_i^0$, around a single adversarial perturbation. SABR [cite] shows that this method is sufficient and produces SOTA results for certified training. For images and other high-dimensional application areas, we expect that there will not be a lot of overlap between these boxes. For a given input $\mathbf{x}_i$ if a perturbation box $b_j^0$ is not adversarial then we will not incur much regularization. If $b_j^0$ is adversarial for $\mathbf{x}_i$ then $b_j^0$ is adversarial for both $\mathbf{x}_i$ and $\mathbf{x}_j$ and thus contains a region which is universally adversarial for both inputs. 





% \begin{itemize}
%     \item SABR shows that optimizing on these small regions is a good proxy for robustness for that input, i.e. these small boxes are good representations of the adversarial examples for that input, therefore good for other boxes to be robust against
%     \item Not optimizing for your own adversarial regions means that we contend less with the standard accuracy/robustness tradeoff. We ultimately are saying that we don't care about single-input robustness only that we do not have a UAP on the batch
%     i
% \end{itemize}

% \begin{figure*}[t]
%     \centering
% \includegraphics[width=1\textwidth]{images/certuap_overview.png}
%     \caption{Overview of \method Training. Each input is shown as an $l_\infty$ ball split into correctly classified region in green ($\greenbox$) and incorrectly classified region in red ($\redbox$). We first compute an adversarial example ($\times$) for each input in the batch and generate a small box ($\square$) around each $\times$, $b_i^0$. Each input is now trained for boxes from all other inputs. We show this propagation for $x_0$. Compared to IBP propagation ($\dashedbox$) we induce much less regularization (big blue <> vs. small blue <>). Depending on the size of the shared region, SABR ($\color{gray}{\dashedbox}$) incurs more regularization (medium blue <>). Before training on the batch there are regions in the perturbation space which are adversarial for multiple inputs (i.e. UAPs), shown by the dark red region ($\darkredbox$). After training, we see that there are still adversarial regions but the shared region no longer exists. }
%     \label{fig:overview}
% \end{figure*}

% \subsection{Overview}

% If a network contained no single-input adversarial perturbations for a ball, $\mathcal{B}(0,\epsilon)$, then there also does not exist any UAPs on the same ball. While we would ideally like to train a network that satisfies the above, existing research has already shown the difficulty of that problem. For worst-case UAP accuracy, the next best scenario is that there only exists single-input adversarial perturbations. This is the key insight of \method. For a given input, it is okay to have an adversarial example, but we want to make sure we do not misclassify on the adversarial examples of other inputs.

% We illustrate this training process in Figure \ref{fig:overview}. SABR shows us that propagating the entire input region ($\dashedbox$) leads to over-approximation of the worst-case loss and thus over-regularization (big blue <>). SABR captures an unsound but much more precise region ($\color{gray}{\dashedbox}$); however, for UAPs, we do not necessarily care that individual adversarial regions exist rather that there are no common regions shared among many inputs. Thus, for the UAP threat model, SABR's box is still over-regularizing (medium blue <>).

% \method propagates the adversarial regions coming from other inputs in the batch. Especially in high dimensional cases like vision, we expect that there will rarely be overlap between two inputs adversarial regions. For example, in Figure \ref{fig:overview}, we propagate $\mathbf{x}_0$ with adversarial regions $b_1, \dots, b_m$ from $\mathbf{x}_1, \dots, \mathbf{x}_m$ respectively. In our example, $b_1$ is not adversarial for $\mathbf{x}_0$ and after propagation we will find that it is already safe for $x_0$ thus leading to significantly less regularization. If there is an overlap in adversarial regions that indicates a high probability of having a UAP which affects both inputs. This is the case for $b_m$ affecting $\mathbf{x}_0$. Depending on the amount of overlap we expect that there is still less regularization than SABR; however, in the case where there is a high level of overlap we want to train to be safe on that region as it has a high chance of affecting more than one input.



==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
